Morphing-based Compression for Data-centric ML Pipelines

Data-centric ML pipelines extend traditional machine learning (ML) pipelines -- of feature transformations and ML model training -- by outer loops for data cleaning, augmentation, and feature engineering to create high-quality input data. Existing lossless matrix compression applies lightweight compression schemes to numeric matrices and performs linear algebra operations such as matrix-vector multiplications directly on the compressed representation but struggles to efficiently rediscover structural data redundancy. Compressed operations are effective at fitting data in available memory, reducing I/O across the storage-memory-cache hierarchy, and improving instruction parallelism. The applied data cleaning, augmentation, and feature transformations provide a rich source of information about data characteristics such as distinct items, column sparsity, and column correlations. In this paper, we introduce BWARE -- an extension of AWARE for workload-aware lossless matrix compression -- that pushes compression through feature transformations and engineering to leverage information about structural transformations. Besides compressed feature transformations, we introduce a novel technique for lightweight morphing of a compressed representation into workload-optimized compressed representations without decompression. BWARE shows substantial end-to-end runtime improvements, reducing the execution time for training data-centric ML pipelines from days to hours.

==> fig/prim/CFrameOrFrame.tex <==

\begin{tikzpicture}
    \node(CFFLLL) at(0, 1){Either};
    \node[bbt1](FFFF)at(-0.15, 0.15){\input{fig/prim/frame.tex}};
    \node[bbt1](CCFFF)at(0.15, -0.15){\input{fig/prim/Cframe.tex}};
    
\end{tikzpicture}


==> fig/prim/CSchemeAndMatrix.tex <==

\begin{tikzpicture}
    \node(CLLL) at(0, 1){And};
    \node[bbt1](CMMM)at(-0.15, 0.15){\input{fig/prim/CScheme.tex}};
    \node[bbt1](CFFF)at(0.15, -0.15){\input{fig/prim/Matrix.tex}};
    
\end{tikzpicture}


==> fig/prim/CmatrixOrFrame.tex <==

\begin{tikzpicture}
    \node(CLLL) at(0, 1){Either};
    \node[bbt1](CMMM)at(-0.15, 0.15){\input{fig/prim/Cmatrix.tex}};
    \node[bbt1](CFFF)at(0.15, -0.15){\input{fig/prim/CFrame.tex}};
    
\end{tikzpicture}


==> fig/prim/algo.tex <==



\lstset{basicstyle=\footnotesize\ttfamily,breaklines=true}


\begin{tikzpicture}[ampersand replacement=\&]

    \node[ inner sep = 0.03cm, minimum height=0.985cm, yshift=0.015cm]{
			% \vspace{-0.3cm}

\begin{lstlisting}
while(){
 q=X%*%p
}
\end{lstlisting}
};

\node at(0,0.7){Algorithm};
\node at(0, -0.46){\ };
\end{tikzpicture}



==> fig/prim/disk.tex <==


\begin{tikzpicture}[ampersand replacement=\&]
    \node{
        \resizebox{0.5cm}{0.5cm}
        {
            \begin{tikzpicture}[ampersand replacement=\&]
                \node{\includegraphics[width = 1cm]{img/Disk.pdf}};
            \end{tikzpicture}
        }
    };
    \node[] at(0,0.35){\fontsize{5pt}{5pt}\textbf{Disk}};
\end{tikzpicture}


==> fig/prim/diskBig.tex <==


\begin{tikzpicture}[ampersand replacement=\&]
    \node{
        \resizebox{1cm}{1cm}
        {
            \begin{tikzpicture}[ampersand replacement=\&]
                \node{\includegraphics[width = 1cm]{img/Disk.pdf}};
            \end{tikzpicture}
        }
    };
    \node[] at(0,0.7){Disk};
\end{tikzpicture}


==> fig/prim/matrix.tex <==
\begin{tikzpicture}[ampersand replacement=\&]
		\node{
				\resizebox{1cm}{1cm}
				{
						\begin{tikzpicture}[ampersand replacement=\&]
								\node[fulln,
										minimum height=4em,
										minimum width=4em]{\ };
						\end{tikzpicture}
				}
		};
		\node at(0,0.7){Matrix};
\end{tikzpicture}

==> fig/prim/matrixOrFrame.tex <==

\begin{tikzpicture}
    \node(LLL) at(0, 1){Either};
    \node[bbt1](MMM)at(-0.15, 0.15){\input{fig/prim/matrix.tex}};
    \node[bbt1](FFF)at(0.15, -0.15){\input{fig/prim/frame.tex}};
    
\end{tikzpicture}


==> fig/prim/morph.tex <==






\begin{tikzpicture}[]
    \node{
        \resizebox{1.106cm}{1cm}
        {
        \includesvg{fig/Bware_350x350.svg}
        }
    };
    \node at(0,0.66){Morph};
\end{tikzpicture}

==> fig/prim/trainLoop.tex <==

\begin{lstlisting}[
	basicstyle=\scriptsize,
]
F = readFrame($1), y = read($2);
for(t : Transformations):
  X = Transform(F, t);
  for(a : ML_Algorithms):
    train(a, X, y);
\end{lstlisting}

